Lexara: A User-Centered Toolkit for Evaluating Large Language Models for Conversational Visual Analytics

Large Language Models (LLMs) are transforming Conversational Visual Analytics (CVA) by enabling data analysis through natural language. However, evaluating LLMs for CVA remains a challenge: requiring programming expertise, overlooking real-world complexity, and lacking interpretable metrics for multi-format (visualizations and text) outputs. Through interviews with 22 CVA developers and 16 end-users, we identified use cases, evaluation criteria and workflows. We present Lexara, a user-centered evaluation toolkit for CVA that operationalizes these insights into: (i) test cases spanning real-world scenarios; (ii) interpretable metrics covering visualization quality (data fidelity, semantic alignment, functional correctness, design clarity) and language quality (factual grounding, analytical reasoning, conversational coherence) using rule-based and LLM-as-a-Judge methods; and (iii) an interactive toolkit enabling experimental setup and multi-format and multi-level exploration of results without programming expertise. We conducted a two-week diary study with six CVA developers, drawn from our initial cohort of 22. Their feedback demonstrated Lexara's effectiveness for guiding appropriate model and prompt selection.

==> 09_acknowledgements.tex <==
\begin{acks}
We thank Yash Tyagi, Kate Mann, Jon Hendrich, and Edouard Picot for their support and feedback. We are grateful to all study participants for their time, insights, and engagement. We also thank the anonymous reviewers for their constructive feedback and suggestions, which helped strengthen this paper.
\end{acks}



